Computing the Thurston-Bennequin invariant in open books

We give explicit formulas and algorithms for the computation of the Thurston-Bennequin invariant of a nullhomologous Legendrian knot on a page of a contact open book and on contact Heegaard surfaces. Furthermore, we extend the results to rationally nullhomologous knots in arbitrary 3-manifolds.

==> knot_complement.tex <==
\section{Appendix}

\begin{lemma}
Let $K$ be a nullhomologous knot in a $3$-manifold $M$. Then
$$
H_1 (M\setminus K) \cong H_1 (M) \oplus \Z,
$$
where the $\Z$-summand is generated by a meridian of $K$.
\end{lemma}

\begin{proof}
Consider the Mayer-Vietoris sequence of the decomposition $M = (M \setminus \nu K) \cup \nu K$. Observe that
$$H_1 (\partial\nu K) \cong H_1 (T^2) \cong  \Z \oplus \Z,$$
generated by a meridian $\mu$ and any longitude $\lambda$ of $K$. Furthermore we have $H_1(\nu K) \cong H_1(K) \cong \Z$.
Since we can assume $M$ to be connected we get a long exact sequence
$$
\cdots \rightarrow H_2(M) \stackrel{\Delta}{\rightarrow} \Z_\mu \oplus \Z_\lambda \stackrel{\alpha}{\rightarrow} H_1(M\setminus K) \oplus \Z \rightarrow H_1(M) \rightarrow 0.
$$
We can represent any generator $f$ of $H_2(M)$ by an embedded surface $F$ transverse to $K$. The boundary homomorphism $\Delta$ thus takes $f$ to a multiple of the meridian:
$$
\Delta (f) = [ F\cap \partial\nu K ] = k_f \mu.
$$ 
Hence, the image of $\Delta$ is of the form $k\mu \oplus 0$ for some $k\in\Z$. By exactness $(k\mu, 0)$ is in the kernel of $\alpha$.
But $K$ is nullhomologous, so it bounds a surface $\Sigma$. The meridian $\mu$ intersects $\Sigma$ in exactly one point, i.e.\ it cannot be a torsion element in $H_1(M\setminus K)$. Therefore $k = 0$ and we get a short exact sequence
$$
0 \rightarrow \Z_\mu \oplus \Z_\lambda \stackrel{\alpha}{\rightarrow} H_1(M\setminus K) \oplus \Z \rightarrow H_1(M) \rightarrow 0.
$$
Furthermore, we can choose the longitude $\lambda$ to be the Seifert longitude. We then have $\alpha (\lambda) = (0,1)$ and as we $\mu$ is trivial in $H_1(\nu K)$, we can reduce the sequence to
$$
0 \rightarrow \Z_\mu \rightarrow H_1(M\setminus K) \rightarrow H_1(M) \rightarrow 0.
$$
The claim follows because the sequence splits. Indeed, the intersection pairing with the class of the Seifert surface yields the desired homomorphism from $H_1(M\setminus K)$ to $\Z_mu$.
\end{proof}

==> thm_env.tex <==
%------------------------------------------------------------
% Theorem like environments
%
\newtheorem{theorem}{Theorem}[section]
\theoremstyle{plain}
\newtheorem{acknowledgement}[theorem]{Acknowledgement}
%\newtheorem{algorithm}[theorem]{Algorithm}
\newtheorem{axiom}[theorem]{Axiom}
\newtheorem{case}[theorem]{Case}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{conclusion}[theorem]{Conclusion}
\newtheorem{condition}[theorem]{Condition}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{criterion}[theorem]{Criterion}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{notation}[theorem]{Notation}
\newtheorem{problem}[theorem]{Problem}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{solution}[theorem]{Solution}
\newtheorem{summary}[theorem]{Summary}
\newtheorem*{result}{Main Result}
% Titel kursiv und nicht fett
%\theoremstyle{remark}
% Titel fett und Inhalt nicht kursiv
\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{algorithm}[theorem]{Algorithm}
\numberwithin{equation}{section}

